AutoFish: Dataset and Benchmark for Fine-grained Analysis of Fish

Automated fish documentation processes are in the near future expected to play an essential role in sustainable fisheries management and for addressing challenges of overfishing. In this paper, we present a novel and publicly available dataset named AutoFish designed for fine-grained fish analysis. The dataset comprises 1,500 images of 454 specimens of visually similar fish placed in various constellations on a white conveyor belt and annotated with instance segmentation masks, IDs, and length measurements. The data was collected in a controlled environment using an RGB camera. The annotation procedure involved manual point annotations, initial segmentation masks proposed by the Segment Anything Model (SAM), and subsequent manual correction of the masks. We establish baseline instance segmentation results using two variations of the Mask2Former architecture, with the best performing model reaching an mAP of 89.15%. Additionally, we present two baseline length estimation methods, the best performing being a custom MobileNetV2-based regression model reaching an MAE of 0.62cm in images with no occlusion and 1.38cm in images with occlusion. Link to project page: https://vap.aau.dk/autofish/.

==> sections/conclusion.tex <==
In this work, we address the gap in data from the fishing industry by introducing \textit{AutoFish}; a dataset comprising 1500 images, aimed at fine-grained analysis for fish, characteristic of the waters around Denmark. It was collected in a lab environment closely resembling the conveyor belt setups one finds in fishing vessels, and is the first dataset to include multiple instances of the same fish, with unique IDs in different positions and orientations. It is additionally thoroughly annotated with detailed segmentation masks, species labels as well as lengths. Alongside the dataset, we present baseline results of instance segmentation and two different approaches to length estimation. Our experiments indicate that even in cases of overlap and occlusion, the state-of-the-art segmentation model \textit{Mask2Former} can achieve very high accuracy, with an average mAP of 89.15\%. Utilizing the predicted masks, a skeletonization approach to length estimation (\textit{SKL}) is capable of accurately estimating fish length with an error of 1.87\% for cases of no occlusion and 4.59\% for the entire dataset. Overcoming the occlusion challenges, the CNN-based regressor (\textit{REG}) estimates length with an error of 3.10\%.
